Splittings of generalized Baumslag-Solitar groups

We study the structure of generalized Baumslag-Solitar groups from the point of view of their (usually non-unique) splittings as fundamental groups of graphs of infinite cyclic groups. We find and characterize certain decompositions of smallest complexity (`fully reduced' decompositions) and give a simplified proof of the existence of deformations. We also prove a finiteness theorem and solve the isomorphism problem for generalized Baumslag-Solitar groups with no non-trivial integral moduli.

==> pics/IAfold.tex <==
\thicklines
\put(10,10){\circle*{1}}
\put(25,15){\circle*{1}}
\put(25,5){\circle*{1}}

%\qbezier(10,10)(10,10)(25,15)
\put(10,10){\line(3,1){15}}
%\qbezier(10,10)(10,10)(25,5)
\put(10,10){\line(3,-1){15}}

\scriptsize
\zindex{12}{12.5}{lm}
\zindex{12}{8}{m}
\zindex{22.5}{15.5}{1}
\zindex{22.5}{4.5}{n}

\put(70,10){\circle*{1}}
\put(86,10){\circle*{1}}

%\qbezier(70,10)(70,10)(86,10)
\put(70,10){\line(1,0){16}}
\zindex{72}{11.3}{m}
\zindex{84.5}{11.3}{n}

\thinlines
\put(45,10){\vector(1,0){10}}

%\qbezier(25,15)(25,15)(29,19)
\put(25,15){\line(1,1){4}}
%\qbezier(25,15)(25,15)(31,16)
\put(25,15){\line(6,1){6}}
%\qbezier(25,5)(25,5)(31,4)
\put(25,5){\line(6,-1){6}}
%\qbezier(25,5)(25,5)(29,1)
\put(25,5){\line(1,-1){4}}

\zindex{31}{19}{r_1}
\zindex{33}{16}{r_2}
\zindex{33}{3.5}{s_1}
\zindex{31}{0.5}{s_2}

%\qbezier(86,10)(86,10)(90,14)
\put(86,10){\line(1,1){4}}
%\qbezier(86,10)(86,10)(92,11)
\put(86,10){\line(6,1){6}}
%\qbezier(86,10)(86,10)(92,9)
\put(86,10){\line(6,-1){6}}
%\qbezier(86,10)(86,10)(90,6)
\put(86,10){\line(1,-1){4}}

\zindex{93.5}{14.5}{lnr_1}
\zindex{95.5}{11.5}{lnr_2}
\zindex{94}{8.5}{s_1}
\zindex{92}{5.5}{s_2}



==> pics/IBexpanded.tex <==
 

==> pics/IBfold.tex <==
\thicklines
\put(10,10){\circle*{1}}
\put(25,15){\circle*{1}}
\put(25,5){\circle*{1}}

%\qbezier(10,10)(10,10)(25,15)
\put(10,10){\line(3,1){15}}
%\qbezier(10,10)(10,10)(25,5)
\put(10,10){\line(3,-1){15}}

\scriptsize
\zindex{12}{12.5}{lm}
\zindex{12}{7.5}{nm}
\zindex{22.5}{15.5}{1}
\zindex{22.5}{4.5}{1}

\put(70,10){\circle*{1}}
\put(86,10){\circle*{1}}

%\qbezier(70,10)(70,10)(86,10)
\put(70,10){\line(1,0){16}}
\zindex{72}{11.3}{m}
\zindex{84.5}{11.3}{1}

\thinlines
\put(45,10){\vector(1,0){10}}

%\qbezier(25,15)(25,15)(29,19)
\put(25,15){\line(1,1){4}}
%\qbezier(25,15)(25,15)(31,16)
\put(25,15){\line(6,1){6}}
%\qbezier(25,5)(25,5)(31,4)
\put(25,5){\line(6,-1){6}}
%\qbezier(25,5)(25,5)(29,1)
\put(25,5){\line(1,-1){4}}

\zindex{31}{19}{r_1}
\zindex{33}{16}{r_2}
\zindex{33}{3.5}{s_1}
\zindex{31}{0.5}{s_2}

%\qbezier(86,10)(86,10)(90,14)
\put(86,10){\line(1,1){4}}
%\qbezier(86,10)(86,10)(92,11)
\put(86,10){\line(6,1){6}}
%\qbezier(86,10)(86,10)(92,9)
\put(86,10){\line(6,-1){6}}
%\qbezier(86,10)(86,10)(90,6)
\put(86,10){\line(1,-1){4}}

\zindex{92.5}{14.5}{lr_1}
\zindex{94.5}{11.5}{lr_2}
\zindex{95}{8.5}{ns_1}
\zindex{93}{5.5}{ns_2}


==> pics/ICfold.tex <==
\thicklines
\put(10,10){\circle{10}}
\put(10,15){\circle*{1}}
\put(25,20){\circle*{1}}
%\qbezier(10,15)(10,15)(25,20)
\put(10,15){\line(3,1){15}}

\put(78,10){\circle{10}}
\put(78,15){\circle*{1}}

\thinlines
\put(45,10){\vector(1,0){10}}

%\qbezier(25,20)(25,20)(29,24)
\put(25,20){\line(1,1){4}}
%\qbezier(25,20)(25,20)(31,21)
\put(25,20){\line(6,1){6}}
%\qbezier(10,15)(10,15)(6,19)
\put(10,15){\line(-1,1){4}}
%\qbezier(10,15)(10,15)(4,16)
\put(10,15){\line(-6,1){6}}

\zindex{31}{24}{r_1}
\zindex{33}{21}{r_2}
\zindex{4.5}{19.5}{s_1}
\zindex{2}{16.5}{s_2}
\zindex{12.5}{17.8}{lm}
\zindex{23}{21}{1}
\zindex{8}{13}{n}
\zindex{12}{13}{m}

%\qbezier(78,15)(78,15)(82,19)
\put(78,15){\line(1,1){4}}
%\qbezier(78,15)(78,15)(84,16)
\put(78,15){\line(6,1){6}}
%\qbezier(78,15)(78,15)(74,19)
\put(78,15){\line(-1,1){4}}
%\qbezier(78,15)(78,15)(72,16)
\put(78,15){\line(-6,1){6}}

\zindex{85.5}{19.5}{lnr_1}
\zindex{87.5}{16.5}{lnr_2}
\zindex{72.5}{19.5}{s_1}
\zindex{70}{16.5}{s_2}
\zindex{76}{13}{n}
\zindex{80}{13}{m}


==> pics/IDexpanded.tex <==
\thicklines
\put(10,15){\circle{10}}
\put(10,10){\circle*{1}}
\put(25,5){\circle*{1}}
%\qbezier(10,10)(10,10)(25,5)
\put(10,10){\line(3,-1){15}}

\put(65,10){\circle*{1}}
\put(80,5){\circle*{1}}
%\qbezier(65,10)(65,10)(80,5)
\put(65,10){\line(3,-1){15}}
\qbezier(65,10)(78,24)(80,5)

\thinlines
\put(40,10){\vector(1,0){10}}
\zindex{45}{12}{\mbox{slide}}

%\qbezier(25,5)(25,5)(29,1)
\put(25,5){\line(1,-1){4}}
%\qbezier(25,5)(25,5)(31,4)
\put(25,5){\line(6,-1){6}}
%\qbezier(10,10)(10,10)(6,6)
\put(10,10){\line(-1,-1){4}}
%\qbezier(10,10)(10,10)(4,9)
\put(10,10){\line(-6,-1){6}}

%\qbezier(80,5)(80,5)(84,1)
\put(80,5){\line(1,-1){4}}
%\qbezier(80,5)(80,5)(86,4)
\put(80,5){\line(6,-1){6}}
%\qbezier(65,10)(65,10)(61,6)
\put(65,10){\line(-1,-1){4}}
%\qbezier(65,10)(65,10)(59,9)
\put(65,10){\line(-6,-1){6}}

\zindex{31}{0.5}{s_1}
\zindex{33}{4}{s_2}
\zindex{4.5}{5.5}{r_1}
\zindex{2}{8.5}{r_2}
\zindex{12}{7.7}{m}
\zindex{22.5}{4.5}{n}
\zindex{8.5}{12}{1}
\zindex{17}{12}{lm}

\zindex{86}{0.5}{s_1}
\zindex{88}{4}{s_2}
\zindex{59.5}{5.5}{r_1}
\zindex{57}{8.5}{r_2}
\zindex{67}{7.7}{m}
\zindex{77.5}{4.5}{n}
\zindex{65.5}{13}{1}
\zindex{82}{8}{ln}


==> pics/IDexpanded2.tex <==
\thicklines
\put(25,10){\circle*{1}}
\put(40,5){\circle*{1}}
\qbezier(25,10)(38,24)(40,5)
\put(35.66987,2.5){\circle{10}}

\put(85,5){\circle{10}}
\put(85,10){\circle*{1}}

\thinlines
\put(0,10){\vector(1,0){10}}
\zindex{5}{12}{\mbox{slide}}

%\qbezier(40,5)(40,5)(44,1)
\put(40,5){\line(1,-1){4}}
%\qbezier(40,5)(40,5)(46,4)
\put(40,5){\line(6,-1){6}}
%\qbezier(25,10)(25,10)(21,6)
\put(25,10){\line(-1,-1){4}}
%\qbezier(25,10)(25,10)(19,9)
\put(25,10){\line(-6,-1){6}}

\zindex{46}{0.5}{s_1}
\zindex{48}{4}{s_2}
\zindex{19.5}{5.5}{r_1}
\zindex{17}{8.5}{r_2}
\zindex{35.6}{9}{lmn}
\zindex{39}{2.5}{n}
\zindex{25.5}{13}{1}
\zindex{42}{8}{ln}

\put(54,10){\vector(1,0){12}}
\zindex{60}{12}{\mbox{collapse}}

%\qbezier(85,10)(85,10)(89,14)
\put(85,10){\line(1,1){4}}
%\qbezier(85,10)(85,10)(91,11)
\put(85,10){\line(6,1){6}}
%\qbezier(85,10)(85,10)(81,14)
\put(85,10){\line(-1,1){4}}
%\qbezier(85,10)(85,10)(79,11)
\put(85,10){\line(-6,1){6}}

\zindex{91}{14.5}{s_1}
\zindex{93}{11.5}{s_2}
\zindex{77.5}{14.5}{lnr_1}
\zindex{75.5}{11.5}{lnr_2}
\zindex{77.5}{8.3}{lmn}
\zindex{87}{8}{n}


==> pics/IDfold.tex <==
\thicklines
\put(10,15){\circle{10}}
\put(10,10){\circle*{1}}
\put(25,5){\circle*{1}}
%\qbezier(10,10)(10,10)(25,5)
\put(10,10){\line(3,-1){15}}

\put(78,15){\circle{10}}
\put(78,10){\circle*{1}}

\thinlines
\put(45,10){\vector(1,0){10}}

%\qbezier(25,5)(25,5)(29,1)
\put(25,5){\line(1,-1){4}}
%\qbezier(25,5)(25,5)(31,4)
\put(25,5){\line(6,-1){6}}
%\qbezier(10,10)(10,10)(6,6)
\put(10,10){\line(-1,-1){4}}
%\qbezier(10,10)(10,10)(4,9)
\put(10,10){\line(-6,-1){6}}

\zindex{31}{0.5}{s_1}
\zindex{33}{4}{s_2}
\zindex{4.5}{5.5}{r_1}
\zindex{2}{8.5}{r_2}
\zindex{12}{7.7}{m}
\zindex{22.5}{4.5}{n}
\zindex{8.5}{12}{1}
\zindex{17}{12}{lm}

%\qbezier(78,10)(78,10)(82,6)
\put(78,10){\line(1,-1){4}}
%\qbezier(78,10)(78,10)(84,9)
\put(78,10){\line(6,-1){6}}
%\qbezier(78,10)(78,10)(74,6)
\put(78,10){\line(-1,-1){4}}
%\qbezier(78,10)(78,10)(72,9)
\put(78,10){\line(-6,-1){6}}

\zindex{84}{5.5}{s_1}
\zindex{86}{8.5}{s_2}
\zindex{71.5}{5.5}{lnr_1}
\zindex{69}{8.5}{lnr_2}
\zindex{76.5}{12}{n}
\zindex{85.5}{12}{lmn}


==> pics/IEexpanded.tex <==
\thicklines
\put(10,10){\circle{10}}
\put(10,15){\circle*{1}}
\put(25,20){\circle*{1}}
%\qbezier(10,15)(10,15)(25,20)
\put(10,15){\line(3,1){15}}

\put(60,15){\circle*{1}}
\put(75,15){\circle*{1}}
\put(90,20){\circle*{1}}
%\qbezier(60,15)(60,15)(75,15)
\put(60,15){\line(1,0){15}}
\qbezier(60,15)(67.5,0)(75,15)
\zindex{67.5}{16}{{\bf e}}
%\qbezier(75,15)(75,15)(90,20)
\put(75,15){\line(3,1){15}}
\zindex{67.5}{9}{{\bf c}}

\thinlines
\put(35,10){\vector(1,0){14}}
\zindex{42}{12}{\mbox{expand }{\bf e}}

%\qbezier(25,20)(25,20)(29,24)
\put(25,20){\line(1,1){4}}
%\qbezier(25,20)(25,20)(31,21)
\put(25,20){\line(6,1){6}}
%\qbezier(10,15)(10,15)(6,19)
\put(10,15){\line(-1,1){4}}
%\qbezier(10,15)(10,15)(4,16)
\put(10,15){\line(-6,1){6}}

%\qbezier(90,20)(90,20)(94,24)
\put(90,20){\line(1,1){4}}
%\qbezier(90,20)(90,20)(96,21)
\put(90,20){\line(6,1){6}}
%\qbezier(60,15)(60,15)(56,19)
\put(60,15){\line(-1,1){4}}
%\qbezier(60,15)(60,15)(54,16)
\put(60,15){\line(-6,1){6}}

\zindex{31}{24}{r_1}
\zindex{33}{21}{r_2}
\zindex{4.5}{19.5}{s_1}
\zindex{2}{16.5}{s_2}
\zindex{12.5}{17.8}{lm}
\zindex{23}{21}{1}
\zindex{8}{13}{1}
\zindex{17}{13}{nm}

\zindex{96}{24}{r_1}
\zindex{98}{21}{r_2}
\zindex{54.5}{19.5}{s_1}
\zindex{52}{16.5}{s_2}
\zindex{76.5}{17}{l}
\zindex{88}{21}{1}
\zindex{60}{12.5}{1}
\zindex{76}{13}{n}
\zindex{62}{16.5}{m}
\zindex{73}{16.5}{1}


==> pics/IEexpanded2.tex <==
\thicklines
\put(30,10){\circle{10}}
\put(30,15){\circle*{1}}
\put(45,20){\circle*{1}}
%\qbezier(30,15)(30,15)(45,20)
\put(30,15){\line(3,1){15}}

\put(85,10){\circle{10}}
\put(85,15){\circle*{1}}

\thinlines
\put(54,10){\vector(1,0){12}}
\zindex{60}{12}{\mbox{collapse}}

\put(0,10){\vector(1,0){14}}
\zindex{7}{12}{\mbox{collapse }{\bf c}}

%\qbezier(45,20)(45,20)(49,24)
\put(45,20){\line(1,1){4}}
%\qbezier(45,20)(45,20)(51,21)
\put(45,20){\line(6,1){6}}
%\qbezier(30,15)(30,15)(26,19)
\put(30,15){\line(-1,1){4}}
%\qbezier(30,15)(30,15)(24,16)
\put(30,15){\line(-6,1){6}}

\zindex{51}{24}{r_1}
\zindex{53}{21}{r_2}
\zindex{23.5}{19.5}{ns_1}
\zindex{21}{16.5}{ns_2}
\zindex{32}{17.5}{l}
\zindex{43}{21}{1}
\zindex{28}{13}{1}
\zindex{37}{13}{nm}

%\qbezier(85,15)(85,15)(89,19)
\put(85,15){\line(1,1){4}}
%\qbezier(85,15)(85,15)(91,16)
\put(85,15){\line(6,1){6}}
%\qbezier(85,15)(85,15)(81,19)
\put(85,15){\line(-1,1){4}}
%\qbezier(85,15)(85,15)(79,16)
\put(85,15){\line(-6,1){6}}

\zindex{92}{19.5}{lr_1}
\zindex{94}{16.5}{lr_2}
\zindex{78.5}{19.5}{ns_1}
\zindex{76.5}{16.5}{ns_2}
\zindex{83}{13}{1}
\zindex{92}{13}{nm}





==> pics/IEfold.tex <==
\thicklines
\put(10,10){\circle{10}}
\put(10,15){\circle*{1}}
\put(25,20){\circle*{1}}
%\qbezier(10,15)(10,15)(25,20)
\put(10,15){\line(3,1){15}}

\put(78,10){\circle{10}}
\put(78,15){\circle*{1}}

\thinlines
\put(45,10){\vector(1,0){10}}

%\qbezier(25,20)(25,20)(29,24)
\put(25,20){\line(1,1){4}}
%\qbezier(25,20)(25,20)(31,21)
\put(25,20){\line(6,1){6}}
%\qbezier(10,15)(10,15)(6,19)
\put(10,15){\line(-1,1){4}}
%\qbezier(10,15)(10,15)(4,16)
\put(10,15){\line(-6,1){6}}

\zindex{31}{24}{r_1}
\zindex{33}{21}{r_2}
\zindex{4.5}{19.5}{s_1}
\zindex{2}{16.5}{s_2}
\zindex{12.5}{17.8}{lm}
\zindex{23}{21}{1}
\zindex{8}{13}{1}
\zindex{17}{13}{nm}

%\qbezier(78,15)(78,15)(82,19)
\put(78,15){\line(1,1){4}}
%\qbezier(78,15)(78,15)(84,16)
\put(78,15){\line(6,1){6}}
%\qbezier(78,15)(78,15)(74,19)
\put(78,15){\line(-1,1){4}}
%\qbezier(78,15)(78,15)(72,16)
\put(78,15){\line(-6,1){6}}

\zindex{85}{19.5}{lr_1}
\zindex{87}{16.5}{lr_2}
\zindex{71.5}{19.5}{ns_1}
\zindex{69.5}{16.5}{ns_2}
\zindex{76}{13}{1}
\zindex{85}{13}{nm}
 

==> pics/IIAfold.tex <==
\thicklines
\put(9,10){\circle*{1}}
\put(25,10){\circle*{1}}
%\qbezier(9,10)(9,10)(25,10)
\put(9,10){\line(1,0){16}}

\scriptsize
\zindex{11.5}{11.5}{lm}
\zindex{23.5}{11.5}{1}

\put(70,10){\circle*{1}}
\put(86,10){\circle*{1}}
%\qbezier(70,10)(70,10)(86,10)
\put(70,10){\line(1,0){16}}

\zindex{72}{11.3}{m}
\zindex{84.5}{11.3}{1}

\thinlines
\put(45,10){\vector(1,0){10}}

%\qbezier(25,10)(25,10)(29,14)
\put(25,10){\line(1,1){4}}
%\qbezier(25,10)(25,10)(31,10)
\put(25,10){\line(1,0){6}}
%\qbezier(25,10)(25,10)(29,6)
\put(25,10){\line(1,-1){4}}

\zindex{31}{14.5}{r_1}
\zindex{33}{10}{r_2}
\zindex{31}{5.5}{r_3}

%\qbezier(86,10)(86,10)(90,14)
\put(86,10){\line(1,1){4}}
%\qbezier(86,10)(86,10)(92,10)
\put(86,10){\line(1,0){6}}
%\qbezier(86,10)(86,10)(90,6)
\put(86,10){\line(1,-1){4}}

\zindex{92.5}{14.5}{lr_1}
\zindex{94.5}{10}{lr_2}
\zindex{92.5}{5.5}{lr_3}


==> pics/IIBexpanded.tex <==
\thicklines
\put(10,10){\circle{10}}
\put(10,15){\circle*{1}}

\put(110,10){\circle{10}}
\put(110,15){\circle*{1}}

\put(60,10){\circle{10}}
\put(60,15){\circle*{1}}
\put(60,5){\circle*{1}}

\thinlines
\put(28,10){\vector(1,0){14}}
\put(78,10){\vector(1,0){14}}

%\qbezier(10,15)(10,15)(14,19)
\put(10,15){\line(1,1){4}}
%\qbezier(10,15)(10,15)(6,19)
\put(10,15){\line(-1,1){4}}
%\qbezier(10,15)(10,15)(10,21)
\put(10,15){\line(0,1){6}}

\zindex{10}{22.5}{r_2}
\zindex{16}{20.5}{r_3}
\zindex{4.5}{20.5}{r_1}
\zindex{8}{13}{1}
\zindex{17}{13}{lm}

%\qbezier(110,15)(110,15)(114,19)
\put(110,15){\line(1,1){4}}
%\qbezier(110,15)(110,15)(106,19)
\put(110,15){\line(-1,1){4}}
%\qbezier(110,15)(110,15)(110,21)
\put(110,15){\line(0,1){6}}

\zindex{110}{22.5}{lr_2}
\zindex{116}{20.5}{lr_3}
\zindex{104.5}{20.5}{lr_1}
\zindex{108}{13}{1}
\zindex{117}{13}{lm}
 
%\qbezier(60,15)(60,15)(64,19)
\put(60,15){\line(1,1){4}}
%\qbezier(60,15)(60,15)(56,19)
\put(60,15){\line(-1,1){4}}
%\qbezier(60,15)(60,15)(60,21)
\put(60,15){\line(0,1){6}}

\zindex{60}{22.5}{r_2}
\zindex{66}{20.5}{r_3}
\zindex{54.5}{20.5}{r_1}
\zindex{58}{12.7}{1}
\zindex{62}{12.7}{m}
\zindex{62}{7.3}{1}
\zindex{58}{7.3}{l}

\zindex{53.5}{10}{\mathbf c}
\zindex{66.5}{10}{\mathbf e}
\zindex{35}{12}{\mbox{expand } {\mathbf e}}
\zindex{85}{12}{\mbox{collapse } {\mathbf c}}

==> pics/IIBfold.tex <==
\thicklines
\put(18,10){\circle{10}}
\put(18,15){\circle*{1}}

\put(78,10){\circle{10}}
\put(78,15){\circle*{1}}

\thinlines
\put(45,10){\vector(1,0){10}}

%\qbezier(18,15)(18,15)(22,19)
\put(18,15){\line(1,1){4}}
%\qbezier(18,15)(18,15)(14,19)
\put(18,15){\line(-1,1){4}}
%\qbezier(18,15)(18,15)(18,21)
\put(18,15){\line(0,1){6}}

\zindex{18}{22.5}{r_2}
\zindex{24}{20.5}{r_3}
\zindex{12.5}{20.5}{r_1}
\zindex{16}{13}{1}
\zindex{25}{13}{lm}

%\qbezier(78,15)(78,15)(82,19)
\put(78,15){\line(1,1){4}}
%\qbezier(78,15)(78,15)(74,19)
\put(78,15){\line(-1,1){4}}
%\qbezier(78,15)(78,15)(78,21)
\put(78,15){\line(0,1){6}}

\zindex{78}{22.5}{lr_2}
\zindex{84}{20.5}{lr_3}
\zindex{72.5}{20.5}{lr_1}
\zindex{76}{13}{1}
\zindex{85}{13}{lm}


==> pics/IIIfold.tex <==
\thicklines
\put(14,8){\circle*{1}}
\put(30,8){\circle*{1}}
\qbezier(14,8)(22,16)(30,8)
\qbezier(14,8)(22,0)(30,8)

\put(70,8){\circle*{1}}
\put(86,8){\circle*{1}}
%\qbezier(70,8)(70,8)(86,8)
\put(70,8){\line(1,0){16}}

\thinlines
\put(45,8){\vector(1,0){10}}

\scriptsize
\zindex{10}{8}{\As_{[w]}}
\zindex{22}{14}{\As_{[e]}}
\zindex{22}{2}{\As_{[f]}}
\zindex{34}{8}{\As_{[u]}}

\zindex{66}{8}{\As_{[w]}}
\zindex{93}{8}{(\As_{[u]}, \gamma)}
\zindex{78}{10}{(\As_{[e]},\As_{[f]})}


==> pics/IIIfoldloop.tex <==
\thicklines
\put(22,5){\circle{10}}
\put(22,15){\circle{10}}
\put(22,10){\circle*{1}}

\put(78,10){\circle{10}}
\put(78,15){\circle*{1}}

\thinlines
\put(45,10){\vector(1,0){10}}

\zindex{15.5}{10.5}{\As_{[w]}}
\zindex{30}{17.5}{\As_{[e]}}
\zindex{30}{2}{\As_{[f]}}

\zindex{78}{3}{(\As_{[e]},\As_{[f]})}
\zindex{78}{17.5}{\As_{[w]}}
 

==> pics/IIfold.tex <==
\thicklines
\put(14,5){\circle*{1}}
\put(30,5){\circle*{1}}
%\qbezier(14,5)(14,5)(30,5)
\put(14,5){\line(1,0){16}}

\put(70,5){\circle*{1}}
\put(86,5){\circle*{1}}
%\qbezier(70,5)(70,5)(86,5)
\put(70,5){\line(1,0){16}}

\thinlines
\put(45,5){\vector(1,0){10}}

\scriptsize
\zindex{10}{5}{\As_{[w]}}
\zindex{22}{7}{\As_{[e]}}
\zindex{34}{5}{\As_{[u]}}

\zindex{66}{5}{\As_{[w]}}
\zindex{93}{5}{(\As_{[u]}, \gamma)}
\zindex{78}{7}{(\As_{[e]},\gamma)}


==> pics/IIfoldloop.tex <==
\thicklines
\put(22,10){\circle{10}}
\put(22,15){\circle*{1}}

\put(78,10){\circle{10}}
\put(78,15){\circle*{1}}

\thinlines
\put(45,10){\vector(1,0){10}}

\zindex{22}{3}{\As_{[e]}}
\zindex{22}{17.5}{\As_{[w]}}

\zindex{78}{3}{(\As_{[e]},\gamma)}
\zindex{78}{17.5}{\As_{[w]}}


==> pics/Ifold.tex <==
\thicklines
\put(10,10){\circle*{1}}
\put(25,15){\circle*{1}}
\put(25,5){\circle*{1}}
%\qbezier(10,10)(10,10)(25,15)
\put(10,10){\line(3,1){15}}
%\qbezier(10,10)(10,10)(25,5)
\put(10,10){\line(3,-1){15}}

\put(70,10){\circle*{1}}
\put(86,10){\circle*{1}}
%\qbezier(70,10)(70,10)(86,10)
\put(70,10){\line(1,0){16}}

\thinlines
\put(45,10){\vector(1,0){10}}

\scriptsize
\zindex{6}{10}{\As_{[w]}}
\zindex{29}{15}{\As_{[u]}}
\zindex{29}{4.5}{\As_{[v]}}
\zindex{66}{10}{\As_{[w]}}
\zindex{95}{10}{(\As_{[u]}, \As_{[v]})}

\zindex{17.5}{15}{\As_{[e]}}
\zindex{17}{5.5}{\As_{[f]}}
\zindex{78}{12}{(\As_{[e]},\As_{[f]})}


==> pics/Ifoldloop.tex <==
\thicklines
\put(10,10){\circle{10}}
\put(10,15){\circle*{1}}
\put(25,20){\circle*{1}}
%\qbezier(10,15)(10,15)(25,20)
\put(10,15){\line(3,1){15}}

\put(78,10){\circle{10}}
\put(78,15){\circle*{1}}

\thinlines
\put(45,10){\vector(1,0){10}}

\zindex{10}{3}{\As_{[f]}}
\zindex{8.5}{17.3}{\As_{[v]}}
\zindex{29}{20}{\As_{[u]}}
\zindex{17}{20}{\As_{[e]}}

\zindex{78}{3}{(\As_{[e]},\As_{[f]})}
\zindex{78}{17}{(\As_{[u]},\As_{[v]})}


==> pics/arr1.tex <==
\scriptsize
\thinlines
%\put(7,5){\circle{4.5}}
\put(7,5){\circle{6}}
%\zindex{7}{5}{C}
\put(10,5){\circle*{1}}
\put(20,5){\circle*{1}}
\put(30,5){\circle*{1}}
\put(40,5){\circle*{1}}
\thicklines
%\put(7,5){\circle{6}}
\put(10,5){\line(1,0){10}}
\put(20,5){\line(1,0){10}}
\put(30,5){\line(1,0){10}}
\zindex{15}{6.5}{G}
\zindex{25}{6.5}{B}
\zindex{35}{6.5}{G}

\thinlines
%\put(57,5){\circle{4.5}} 
\put(57,5){\circle{6}} 
%\zindex{57}{5}{C}
\put(60,5){\circle*{1}}
\put(70,5){\circle*{1}}
\put(78,9){\circle*{1}}
\put(78,1){\circle*{1}}
\put(60,5){\line(1,0){10}}
\thicklines
%\put(57,5){\circle{6}}
\put(70,5){\line(2,1){8}}
\put(70,5){\line(2,-1){8}}
\zindex{74}{9}{G}
\zindex{74}{1}{G}

\thinlines
%\put(97,5){\circle{4.5}} 
\put(97,5){\circle{6}} 
%\zindex{97}{5}{C}
\put(100,5){\circle*{1}}
\put(110,5){\circle*{1}}
\put(120,5){\circle*{1}}
\put(108,1){\circle*{1}}
\thicklines
%\put(97,5){\circle{6}}
\put(100,5){\line(1,0){10}}
\put(110,5){\line(1,0){10}}
\put(100,5){\line(2,-1){8}}
\zindex{105}{6.5}{G}
\zindex{115}{6.5}{B}
\zindex{104}{1}{G}


==> pics/arr2.tex <==
\scriptsize
\thinlines
%\put(7,5){\circle{4.5}}
\put(7,5){\circle{6}}
%\zindex{7}{5}{C}
\put(10,5){\circle*{1}}
\put(20,5){\circle*{1}}
\put(30,5){\circle*{1}}
\put(40,5){\circle*{1}}
\put(20,5){\line(1,0){10}}
\thicklines
%\put(7,5){\circle{6}}
\put(10,5){\line(1,0){10}}
\put(30,5){\line(1,0){10}}
\zindex{15}{6.5}{G}
\zindex{35}{6.5}{B}

\thinlines
%\put(57,5){\circle{4.5}} 
\put(57,5){\circle{6}} 
%\zindex{57}{5}{C}
\put(60,5){\circle*{1}}
\put(70,5){\circle*{1}}
\put(78,9){\circle*{1}}
\put(78,1){\circle*{1}}
\put(70,5){\line(2,-1){8}}
\thicklines
%\put(57,5){\circle{6}}
\put(60,5){\line(1,0){10}}
\put(70,5){\line(2,1){8}}
\zindex{65}{6.5}{G}
\zindex{74}{9}{B}

\thinlines
%\put(97,5){\circle{4.5}} 
\put(97,5){\circle{6}} 
%\zindex{97}{5}{C}
\put(100,5){\circle*{1}}
\put(110,5){\circle*{1}}
\put(120,5){\circle*{1}}
\put(108,1){\circle*{1}}
\put(100,5){\line(1,0){10}}
\thicklines
%\put(97,5){\circle{6}}
\put(110,5){\line(1,0){10}}
\put(100,5){\line(2,-1){8}}
\zindex{115}{6.5}{G}
\zindex{104}{1}{G}


==> pics/arr3.tex <==
\scriptsize
\thinlines
%\put(7,5){\circle{4.5}}
\put(7,5){\circle{6}}
%\zindex{7}{5}{C}
\put(10,5){\circle*{1}}
\put(20,5){\circle*{1}}
\put(30,5){\circle*{1}}
\put(40,5){\circle*{1}}
\put(10,5){\line(1,0){10}}
\put(30,5){\line(1,0){10}}
\thicklines
%\put(7,5){\circle{6}}
\put(20,5){\line(1,0){10}}
\zindex{25}{6.5}{G}

\thinlines
%\put(57,5){\circle{4.5}} 
\put(57,5){\circle{6}} 
%\zindex{57}{5}{C}
\put(60,5){\circle*{1}}
\put(70,5){\circle*{1}}
\put(80,5){\circle*{1}}
\put(68,1){\circle*{1}}
\put(70,5){\line(1,0){10}}
\put(60,5){\line(2,-1){8}}
\thicklines
%\put(57,5){\circle{6}}
\put(60,5){\line(1,0){10}}
\zindex{65}{6.5}{G}

\thinlines
%\put(97,5){\circle{4.5}} 
%\put(97,5){\circle{6}} 
\put(96,5){\circle{8}}
\put(92,5){\circle*{1}}
%\zindex{96}{5}{C}
\put(100,5){\circle*{1}}
\put(110,5){\circle*{1}}
\put(120,5){\circle*{1}}
\put(110,5){\line(1,0){10}}
\thicklines
%\put(96,5){\circle{8}} 
\put(100,5){\line(1,0){10}}
\zindex{105}{6.5}{G}




==> pics/arr4.tex <==
\scriptsize
\thinlines
%\put(7,5){\circle{4.5}}
\put(7,5){\circle{6}}
%\zindex{7}{5}{C}
\put(10,5){\circle*{1}}
\put(20,5){\circle*{1}}
\put(18,9){\circle*{1}}
\put(18,1){\circle*{1}}
\put(10,5){\line(1,0){10}}
\thicklines
%\put(7,5){\circle{6}}
\put(10,5){\line(2,1){8}}
\put(10,5){\line(2,-1){8}}
\zindex{14}{9}{G}
\zindex{14}{1}{G}

\thinlines
%\put(57,5){\circle{4.5}}
%\put(57,5){\circle{6}}
\put(56,5){\circle{8}}
\put(52,5){\circle*{1}}
%\zindex{56}{5}{C}
\put(60,5){\circle*{1}}
\put(68,9){\circle*{1}}
\put(68,1){\circle*{1}}
\thicklines
%\put(56,5){\circle{8}}
\put(60,5){\line(2,1){8}}
\put(60,5){\line(2,-1){8}}
\zindex{64}{9}{G}
\zindex{64}{1}{G}

\thinlines
%\put(107,5){\circle{4.5}} 
%\put(107,5){\circle{6}} 
\put(106,5){\circle{8}} 
%\zindex{106}{5}{C}
\put(102,5){\circle*{1}}
\put(92,5){\circle*{1}}
\put(110,5){\circle*{1}}
\put(120,5){\circle*{1}}
\thicklines
%\put(106,5){\circle{8}} 
\put(92,5){\line(1,0){10}}
\put(110,5){\line(1,0){10}}
\zindex{115}{6.5}{G}
\zindex{97}{6.5}{G}
 

==> pics/collapse.tex <==
\thicklines
\put(10,10){\circle*{1}}
\put(25,10){\circle*{1}}
\put(10,10){\line(1,0){15}}

\thinlines
\put(45,10){\vector(1,0){10}}

\put(25,10){\line(5,3){5}}
\put(25,10){\line(5,-3){5}}

\put(10,10){\line(-5,3){5}}
\put(4,10){\line(1,0){6}}
\put(10,10){\line(-5,-3){5}}

\put(75,10){\circle*{1}}
\put(75,10){\line(-5,3){5}}
\put(69,10){\line(1,0){6}}
\put(75,10){\line(-5,-3){5}}

\put(75,10){\line(5,3){5}}
\put(75,10){\line(5,-3){5}}

\scriptsize
\zindex{10}{12.5}{\As_v}
\zindex{17}{11.5}{\As_e}
\zindex{25}{12.5}{\As_e}
\zindex{33}{14}{\As_{e_1}}
\zindex{33}{6}{\As_{e_2}}

\zindex{75}{12.5}{\As_v}
\zindex{83}{14}{\As_{e_1}}
\zindex{83}{6}{\As_{e_2}}



==> pics/countereg1.tex <==
\thicklines
\put(10,10){\circle*{1}}
\put(22,10){\circle*{1}}
\put(5,10){\circle{10}}
%\qbezier(10,10)(10,10)(22,10)
\put(10,10){\line(1,0){12}}
\scriptsize
\zindex{6}{8.5}{mnr}
\zindex{8}{11.5}{r}
\zindex{13.5}{12}{rm^2}
\zindex{20.5}{11.5}{s}

\put(48,5){\circle*{1}}
\put(60,5){\circle*{1}}
\put(72,5){\circle*{1}}
%\qbezier(48,5)(48,5)(72,5)
\put(48,5){\line(1,0){24}}
\qbezier(48,5)(54,20)(60,5)
\zindex{49.5}{3.5}{r}
\zindex{58.5}{3.5}{n}
\zindex{62}{3.5}{m}
\zindex{70.5}{3.5}{s}
\zindex{46}{7}{rm}
\zindex{61}{7}{1}
 
\put(98,5){\circle*{1}}
\put(110,5){\circle*{1}}
\put(122,5){\circle*{1}}
%\qbezier(98,5)(98,5)(122,5)
\put(98,5){\line(1,0){24}}
\put(110,10){\circle{10}}
\zindex{99.5}{3.5}{r}
\zindex{108.5}{3.5}{n}
\zindex{112}{3.5}{m}
\zindex{120.5}{3.5}{s}
\zindex{108.5}{7}{1}
\zindex{117}{7}{mn}

\thinlines
\put(29,10){\vector(1,0){12}}
\zindex{35}{11.5}{\mbox{expand}}

\put(79,10){\vector(1,0){12}}
\zindex{85}{11.5}{\mbox{slide}}


==> pics/countereg2.tex <==
\thicklines
\put(70,10){\circle*{1}}
\put(82,10){\circle*{1}}
\put(87,10){\circle{10}}
%\qbezier(70,10)(70,10)(82,10)
\put(70,10){\line(1,0){12}}
\scriptsize
\zindex{86}{8.5}{mns}
\zindex{84}{11.5}{s}
\zindex{79.5}{12}{sn^2}
\zindex{71.5}{11.5}{r}

\put(20,5){\circle*{1}}
\put(32,5){\circle*{1}}
\put(44,5){\circle*{1}}
%\qbezier(20,5)(20,5)(44,5)
\put(20,5){\line(1,0){24}}
\qbezier(32,5)(38,20)(44,5)
\zindex{21.5}{3.5}{r}
\zindex{30.5}{3.5}{n}
\zindex{34}{3.5}{m}
\zindex{42.5}{3.5}{s}
\zindex{31}{7}{1}
\zindex{46}{7}{ns}

\thinlines
\put(1,10){\vector(1,0){12}}
\zindex{7}{11.5}{\mbox{slide}}

\put(51,10){\vector(1,0){12}}
\zindex{57}{11.5}{\mbox{collapse}}


==> pics/countereg3.tex <==
\thicklines
\put(10,15){\circle*{1}}
\put(22,15){\circle*{1}}
\put(0,15){\circle*{1}}
\put(22,5){\circle*{1}}
\put(5,15){\circle{10}}
\put(10,15){\line(1,0){12}}
\put(22,5){\line(0,1){10}}
\scriptsize
\zindex{6}{17}{mnr}
\zindex{8}{13}{r}
\zindex{-1}{13.5}{z}
\zindex{-1}{16.5}{z}
\zindex{13.5}{17}{rm^2}
\zindex{20.5}{16.5}{s}
\zindex{23.5}{13.5}{s}
\zindex{23.5}{6.5}{z}

\put(60,15){\circle*{1}}
\put(72,15){\circle*{1}}
\put(72,5){\circle*{1}}
\put(60,5){\circle*{1}}
\put(55,15){\circle{10}}
\put(60,15){\line(1,0){12}}
\put(72,5){\line(0,1){10}}
\put(60,5){\line(0,1){10}}
\scriptsize
\zindex{56}{17}{mnr}
\zindex{58}{13}{r}
\zindex{63.5}{17}{rm^2}
\zindex{70.5}{16.5}{s}
\zindex{61.5}{13.5}{r}
\zindex{61.5}{6.5}{z}
\zindex{73.5}{13.5}{s}
\zindex{73.5}{6.5}{z}

\thinlines
\put(29,15){\vector(1,0){12}}
\zindex{35}{16.5}{\mbox{slide}}

\put(79,15){\vector(1,0){12}}
\zindex{85}{16.5}{\mbox{expand}}


==> pics/countereg4.tex <==
\thicklines
\put(-2,15){\circle*{1}}
\put(10,15){\circle*{1}}
\put(22,15){\circle*{1}}
\put(-2,15){\line(1,0){24}}
\qbezier(-2,15)(4,30)(10,15)
\scriptsize
\zindex{-0.5}{13.5}{r}
\zindex{8.5}{13.5}{n}
\zindex{12}{13.5}{m}
\zindex{20.5}{13.5}{s}
\zindex{-4}{17}{rm}
\zindex{11}{17}{1}
\put(-2,5){\circle*{1}}
\put(22,5){\circle*{1}}
\put(-2,5){\line(0,1){10}}
\put(22,5){\line(0,1){10}}
\zindex{-3.5}{13.5}{r}
\zindex{-3.5}{6.5}{z}
\zindex{23.5}{13.5}{s}
\zindex{23.5}{6.5}{z}
 
\put(48,15){\circle*{1}}
\put(60,15){\circle*{1}}
\put(72,15){\circle*{1}}
\put(48,15){\line(1,0){24}}
\put(60,20){\circle{10}}
\zindex{49.5}{13.5}{r}
\zindex{58.5}{13.5}{n}
\zindex{62}{13.5}{m}
\zindex{70.5}{13.5}{s}
\zindex{58.5}{17}{1}
\zindex{67}{17}{mn}
\put(48,5){\circle*{1}}
\put(72,5){\circle*{1}}
\put(48,5){\line(0,1){10}}
\put(72,5){\line(0,1){10}}
\zindex{46.5}{13.5}{r}
\zindex{46.5}{6.5}{z}
\zindex{73.5}{13.5}{s}
\zindex{73.5}{6.5}{z}

\put(98,15){\circle*{1}}
\put(110,15){\circle*{1}}
\put(122,15){\circle*{1}}
\put(98,15){\line(1,0){24}}
\qbezier(110,15)(116,30)(122,15)
\zindex{99.5}{13.5}{r}
\zindex{108.5}{13.5}{n}
\zindex{112}{13.5}{m}
\zindex{120.5}{13.5}{s}
\zindex{109}{17}{1}
\zindex{124}{17}{ns}
\put(98,5){\circle*{1}}
\put(122,5){\circle*{1}}
\put(98,5){\line(0,1){10}}
\put(122,5){\line(0,1){10}}
\zindex{96.5}{13.5}{r}
\zindex{96.5}{6.5}{z}
\zindex{123.5}{13.5}{s}
\zindex{123.5}{6.5}{z}

\thinlines
\put(29,15){\vector(1,0){12}}
\zindex{35}{16.5}{\mbox{slide}}

\put(79,15){\vector(1,0){12}}
\zindex{85}{16.5}{\mbox{slide}}


==> pics/countereg5.tex <==
\thicklines
\put(70,15){\circle*{1}}
\put(82,15){\circle*{1}}
\put(87,15){\circle{10}}
\put(92,15){\circle*{1}}
\put(70,15){\line(1,0){12}}
\scriptsize
\zindex{86}{17}{mns}
\zindex{84}{13}{s}
\zindex{79.5}{17}{sn^2}
\zindex{71.5}{16.5}{r}
\zindex{93}{16.5}{z}
\zindex{93}{13.5}{z}
\put(70,5){\circle*{1}}
\put(70,5){\line(0,1){10}}
\zindex{68.5}{13.5}{r}
\zindex{68.5}{6.5}{z}

\put(20,15){\circle*{1}}
\put(32,15){\circle*{1}}
\put(37,15){\circle{10}}
\put(20,15){\line(1,0){12}}
\scriptsize
\zindex{36}{17}{mns}
\zindex{34}{13}{s}
\zindex{29.5}{17}{sn^2}
\zindex{21.5}{16.5}{r}
\put(20,5){\circle*{1}}
\put(32,5){\circle*{1}}
\put(20,5){\line(0,1){10}}
\put(32,5){\line(0,1){10}}
\zindex{18.5}{13.5}{r}
\zindex{18.5}{6.5}{z}
\zindex{30.5}{13.5}{s}
\zindex{30.5}{6.5}{z}

\thinlines
\put(1,15){\vector(1,0){12}}
\zindex{7}{16.5}{\mbox{collapse}}

\put(51,15){\vector(1,0){12}}
\zindex{57}{16.5}{\mbox{slide}}


==> pics/expand.tex <==
\thicklines
\put(70,10){\circle*{1}}
\put(85,10){\circle*{1}}
\put(70,10){\line(1,0){15}}

\thinlines
\put(45,10){\vector(1,0){10}}

\put(85,10){\line(5,3){5}}
\put(85,10){\line(5,-3){5}}

\put(70,10){\line(-5,3){5}}
\put(64,10){\line(1,0){6}}
\put(70,10){\line(-5,-3){5}}

\put(20,10){\circle*{1}}
\put(20,10){\line(-5,3){5}}
\put(14,10){\line(1,0){6}}
\put(20,10){\line(-5,-3){5}}

\put(20,10){\line(5,3){5}}
\put(20,10){\line(5,-3){5}}

\scriptsize
\zindex{70}{12.5}{\As_v}
\zindex{77}{11.5}{H}
\zindex{85}{12.5}{H}
\zindex{93}{14}{\As_{e_1}}
\zindex{93}{6}{\As_{e_2}}

\zindex{20}{12.5}{\As_v}
\zindex{28}{14}{\As_{e_1}}
\zindex{28}{6}{\As_{e_2}}


==> pics/expcollapseC.tex <==
\scriptsize
\thicklines
\put(10,28){\circle*{1}}
\put(22,28){\circle*{1}}
\put(10,28){\line(1,0){12}}

\put(48,28){\circle*{1}}
\put(60,28){\circle*{1}}
\put(72,28){\circle*{1}}
\put(48,28){\line(1,0){24}}

\put(98,28){\circle*{1}}
\put(110,28){\circle*{1}}
\put(98,28){\line(1,0){12}}

\put(60,8){\circle*{1}}

\thinlines
\put(29,28){\vector(1,0){12}}
\put(79,28){\vector(1,0){12}}
\zindex{35}{29.5}{\mbox{expand}}
\zindex{85}{29.5}{\mbox{collapse}}

\put(10,28){\line(-3,5){3}}
\put(10,28){\line(-3,-5){3}}
\put(22,28){\line(3,5){3}}
\zindex{16}{29.8}{\mathbf e'}
\zindex{12}{26.5}{kl}
\zindex{20.5}{26.5}{1}
\zindex{6.5}{22}{r}
\zindex{6}{34.5}{ks}
\zindex{26}{34}{t}

\put(60,28){\line(-3,5){3}}
\put(48,28){\line(-3,-5){3}}
\put(72,28){\line(3,5){3}}
\zindex{54}{29.3}{\mathbf e}
\zindex{66}{29.8}{\mathbf e'}
\zindex{49.5}{26.5}{k}
\zindex{58.5}{26.5}{1}
\zindex{61.5}{26.5}{l}
\zindex{70.5}{26.5}{1}
\zindex{44.5}{22}{r}
\zindex{56}{34}{s}
\zindex{76}{34}{t}

\put(110,28){\line(-3,5){3}}
\put(98,28){\line(-3,-5){3}}
\put(110,28){\line(3,5){3}}
\zindex{104}{29.3}{\mathbf e}
\zindex{99.5}{26.5}{k}
\zindex{108.5}{26.5}{1}
\zindex{94.5}{22}{r}
\zindex{106}{34}{s}
\zindex{114}{34.5}{lt}
 
\put(60,8){\line(-3,5){3}}
\put(60,8){\line(-3,-5){3}}
\put(60,8){\line(3,5){3}}

\put(31,18){\vector(2,-1){11}}
\put(78,12.5){\vector(2,1){11}}
\zindex{31}{14}{\mbox{collapse}}
\zindex{89}{14}{\mbox{expand}}
\zindex{56.5}{2}{r}
\zindex{56}{14.5}{ks}
\zindex{64}{14.5}{klt}
 

==> pics/expcollapseD.tex <==
\scriptsize
\thicklines
\put(10,28){\circle*{1}}
\put(22,28){\circle*{1}}
\put(10,28){\line(1,0){12}}

\put(48,28){\circle*{1}}
\put(60,28){\circle*{1}}
\put(72,28){\circle*{1}}
\put(48,28){\line(1,0){24}}

\put(98,28){\circle*{1}}
\put(110,28){\circle*{1}}
\put(98,28){\line(1,0){12}}

\put(60,8){\circle*{1}}

\thinlines
\put(29,28){\vector(1,0){12}}
\put(79,28){\vector(1,0){12}}
\zindex{35}{29.5}{\mbox{expand}}
\zindex{85}{29.5}{\mbox{collapse}}

\put(10,28){\line(-3,5){3}}
\put(10,28){\line(-3,-5){3}}
\put(22,28){\line(3,5){3}}
\zindex{16}{29.8}{\mathbf e'}
\zindex{12}{26.5}{1}
\zindex{20.5}{26.5}{l}
\zindex{6.5}{22}{kr}
\zindex{6}{34}{s}
\zindex{26}{34}{t}

\put(60,28){\line(-3,5){3}}
\put(48,28){\line(-3,-5){3}}
\put(72,28){\line(3,5){3}}
\zindex{54}{29.3}{\mathbf e}
\zindex{66}{29.8}{\mathbf e'}
\zindex{49.5}{26.5}{1}
\zindex{58.5}{26.5}{k}
\zindex{61.5}{26.5}{1}
\zindex{70.5}{26.5}{l}
\zindex{44.5}{22}{r}
\zindex{56}{34}{s}
\zindex{76}{34}{t}

\put(110,28){\line(-3,5){3}}
\put(98,28){\line(-3,-5){3}}
\put(110,28){\line(3,5){3}}
\zindex{104}{29.3}{\mathbf e}
\zindex{99.5}{26.5}{1}
\zindex{108}{26.5}{kl}
\zindex{94.5}{22}{r}
\zindex{106}{34.5}{ls}
\zindex{114}{34}{t}
 
\put(60,8){\line(-3,5){3}}
\put(60,8){\line(-3,-5){3}}
\put(60,8){\line(3,5){3}}

\put(31,18){\vector(2,-1){11}}
\put(78,12.5){\vector(2,1){11}}
\zindex{31}{14}{\mbox{collapse}}
\zindex{89}{14}{\mbox{expand}}
\zindex{56.5}{1.5}{klr}
\zindex{56}{14.5}{ls}
\zindex{64}{14}{t}
 

==> pics/expslide2.tex <==
\scriptsize
\thicklines
\put(15,5){\circle*{1}}
\put(15,15){\circle*{1}}
\thinlines
\put(15,5){\line(0,1){10}}
\put(15,5){\line(5,3){5}}
\put(15,5){\line(5,-3){5}}
\put(15,5){\line(-1,0){6}}
\put(15,5){\line(-1,1){4}}
\put(15,5){\line(-1,-1){4}}
\put(15,15){\line(6,1){6}}
\put(15,15){\line(1,1){4}}
%% \zindex{13.5}{10.5}{\mathbf e_1}
\zindex{16.5}{7.8}{l}
\zindex{16.5}{13.5}{k}
\zindex{22}{8.5}{r_1}
\zindex{22}{1.5}{r_2}
\zindex{7}{5}{ls_2}
\zindex{9}{10.5}{ls_1}
\zindex{10}{0}{ls_3}
\zindex{23}{16}{t_2}
\zindex{21}{20}{t_1}

\put(27,10){\vector(1,0){12}}
\zindex{33}{11.5}{\mbox{exp.}}

\thicklines
\put(52,5){\circle*{1}}
\put(52,15){\circle*{1}}
\put(67,5){\circle*{1}}
\put(52,5){\line(1,0){15}}
\thinlines
\put(52,5){\line(0,1){10}}
\put(67,5){\line(5,3){5}}
\put(67,5){\line(5,-3){5}}
\put(52,5){\line(-1,0){6}}
\put(52,5){\line(-1,1){4}}
\put(52,5){\line(-1,-1){4}}
\put(52,15){\line(6,1){6}}
\put(52,15){\line(1,1){4}}
\zindex{74}{8.5}{r_1}
\zindex{74}{1.5}{r_2}
\zindex{44}{5}{s_2}
\zindex{46.5}{10}{s_1}
\zindex{46.5}{0}{s_3}
%% \zindex{50.5}{10.5}{\mathbf e_1}
\zindex{53.5}{7}{1}
\zindex{53.5}{13.5}{k}
%% \zindex{60}{6}{\mathbf e}
\zindex{54}{3.5}{1}
\zindex{65}{3.5}{l}
\zindex{60}{16}{t_2}
\zindex{58}{20}{t_1}

\put(78,10){\vector(1,0){12}}
\zindex{84}{12}{\mbox{slide}}

\thicklines
\put(102,5){\circle*{1}}
\put(102,15){\circle*{1}}
\put(117,5){\circle*{1}}
\put(102,15){\line(3,-2){15}}
\thinlines
\put(102,5){\line(0,1){10}}
\put(117,5){\line(5,3){5}}
\put(117,5){\line(5,-3){5}}
\put(102,5){\line(-1,0){6}}
\put(102,5){\line(-1,1){4}}
\put(102,5){\line(-1,-1){4}}
\put(102,15){\line(1,6){1}}
\put(102,15){\line(1,1){4}}
\zindex{124}{8.5}{r_1}
\zindex{124}{1.5}{r_2}
\zindex{94}{5}{s_2}
\zindex{96.5}{10}{s_1}
\zindex{96.5}{0}{s_3}
%% \zindex{100.5}{10.5}{\mathbf e_1}
\zindex{103.5}{7}{1}
\zindex{103.5}{12.5}{k}
%% \zindex{110.5}{11}{\mathbf e}
\zindex{105}{15}{k}
\zindex{116}{8}{l}
\zindex{104}{22.5}{t_1}
\zindex{107.5}{20}{t_2}




==> pics/expslide3.tex <==
\scriptsize
\thicklines
\put(15,5){\circle*{1}}
\put(15,15){\circle*{1}}
\thinlines
\put(15,5){\line(0,1){10}}
\put(15,5){\line(5,3){5}}
\put(15,5){\line(5,-3){5}}
\put(15,5){\line(-1,0){6}}
\put(15,5){\line(-1,1){4}}
\put(15,5){\line(-1,-1){4}}
\put(15,15){\line(6,1){6}}
\put(15,15){\line(1,1){4}}
%% \zindex{13.5}{10.5}{\mathbf e_1}
\zindex{16.5}{7.8}{l}
\zindex{16.5}{13.5}{k}
\zindex{22}{8.5}{r_1}
\zindex{22}{1.5}{r_2}
\zindex{7}{5}{ls_2}
\zindex{9}{10.5}{ls_1}
\zindex{10}{0}{ls_3}
\zindex{23}{16}{t_2}
\zindex{21}{20}{t_1}

\put(31,10){\vector(1,0){12}}
\zindex{37}{12}{\mbox{slides}}

\thicklines
\put(60,5){\circle*{1}}
\put(60,15){\circle*{1}}
\thinlines
\put(60,5){\line(0,1){10}}
\put(60,5){\line(5,3){5}}
\put(60,5){\line(5,-3){5}}
\put(60,15){\line(-1,0){6}}
\put(60,15){\line(-1,1){4}}
\put(60,15){\line(-1,-1){4}}
\put(60,15){\line(6,1){6}}
\put(60,15){\line(1,1){4}}
\zindex{67}{8.5}{r_1}
\zindex{67}{1.5}{r_2}
\zindex{51.5}{15}{ks_2}
\zindex{54}{20.5}{ks_1}
\zindex{54.5}{10}{ks_3}
%% \zindex{58.5}{10.5}{\mathbf e_1}
\zindex{61.5}{7.8}{l}
\zindex{61.5}{13.5}{k}
\zindex{68}{16}{t_2}
\zindex{66}{20}{t_1}

\put(78,10){\vector(1,0){12}}
\zindex{84}{11.5}{\mbox{exp.}}

\thicklines
\put(102,15){\circle*{1}}
\put(117,15){\circle*{1}}
\put(117,5){\circle*{1}}
\put(102,15){\line(1,0){15}}
\thinlines
\put(117,5){\line(0,1){10}}
\put(117,5){\line(5,3){5}}
\put(117,5){\line(5,-3){5}}
\put(102,15){\line(-1,0){6}}
\put(102,15){\line(-1,1){4}}
\put(102,15){\line(-1,-1){4}}
\put(117,15){\line(6,1){6}}
\put(117,15){\line(1,1){4}}
\zindex{124}{8.5}{r_1}
\zindex{124}{1.5}{r_2}
\zindex{94}{15}{s_2}
\zindex{96.5}{20}{s_1}
\zindex{96.5}{10}{s_3}
%% \zindex{115.5}{10.5}{\mathbf e_1}
\zindex{118.5}{7.8}{l}
\zindex{118.5}{12.5}{k}
%% \zindex{109.5}{16}{\mathbf e}
\zindex{103.5}{16.5}{1}
\zindex{115.5}{16.5}{k}
\zindex{125}{16}{t_2}
\zindex{123}{20}{t_1}


==> pics/fixpath.tex <==
\scriptsize
\thicklines
\put(10,5){\circle*{1}}
\put(30,5){\circle*{1}}
\put(50,5){\circle*{1}}
\put(70,5){\circle*{1}}
\put(10,5){\line(1,0){69}}

\zindex{84}{5}{\cdots}

\zindex{12}{6.5}{\pm 1}
\zindex{27}{6.5}{m_1}
\zindex{33}{6.5}{n_1}
\zindex{47}{6.5}{m_2}
\zindex{53}{6.5}{n_2}
\zindex{67}{6.5}{m_3}
\zindex{73}{6.5}{n_3}

\zindex{20.5}{3.2}{\mathbf e_1}
\zindex{40.5}{3.2}{\mathbf e_2}
\zindex{60.5}{3.2}{\mathbf e_3}

\zindex{10}{2.5}{<\!\gamma\!>}
\zindex{30}{2.5}{<\!\sigma_1\!>}
\zindex{50}{2.5}{<\!\sigma_2\!>}
\zindex{70}{2.5}{<\!\sigma_3\!>}


==> pics/fixpath2.tex <==
\scriptsize
\thicklines
\put(10,5){\circle*{1}}
\put(30,5){\circle*{1}}
\put(50,5){\circle*{1}}
\put(70,5){\circle*{1}}
\put(10,5){\line(1,0){69}}

\zindex{84}{5}{\cdots}

\zindex{12}{6.5}{\pm 1}
\zindex{27}{6.5}{m_1}
\zindex{33}{6.5}{n_1}
\zindex{47}{6.5}{m_2}
\zindex{53}{6.5}{n_2}
\zindex{67}{6.5}{m_3}
\zindex{73}{6.5}{n_3}

\zindex{20.5}{3.2}{\mathbf e_1}
\zindex{40.5}{3.2}{\mathbf e_2}
\zindex{60.5}{3.2}{\mathbf e_3}

\zindex{10}{2.8}{x}
\zindex{30.5}{2.8}{x_1}
\zindex{50.5}{2.8}{x_2}
\zindex{70.5}{2.8}{x_3}


==> pics/fullyred.tex <==
\thicklines
\put(10,10){\circle{10}}
\put(10,15){\circle*{1}}

\put(110,10){\circle{10}}
\put(110,15){\circle*{1}}

\put(60,10){\circle{10}}
\put(60,15){\circle*{1}}
\put(60,5){\circle*{1}}


\thinlines
\put(28,10){\vector(1,0){14}}
\put(78,10){\vector(1,0){14}}
\put(10,15){\line(1,1){4}}
\put(110,15){\line(1,1){4}}
\put(60,15){\line(1,1){4}}

\put(10,15){\line(-1,1){4}}
\put(10,15){\line(0,1){6}}

\zindex{10}{22.5}{r_2}
\zindex{16}{20.5}{r_3}
\zindex{4.5}{20.5}{r_1}
\zindex{8}{13}{1}
\zindex{17}{13}{lm}

\put(110,15){\line(-1,1){4}}
\put(110,15){\line(0,1){6}}

\zindex{110}{22.5}{lr_2}
\zindex{116}{20.5}{lr_3}
\zindex{104.5}{20.5}{lr_1}
\zindex{108}{13}{1}
\zindex{117}{13}{lm}
 
\put(60,15){\line(-1,1){4}}
\put(60,15){\line(0,1){6}}

\zindex{60}{22.5}{r_2}
\zindex{66}{20.5}{r_3}
\zindex{54.5}{20.5}{r_1}
\zindex{58}{12.7}{1}
\zindex{62}{12.7}{m}
\zindex{62}{3.7}{1}
\zindex{58}{3.7}{l}
% \zindex{62}{7.3}{1}
% \zindex{58}{7.3}{l}

\zindex{53}{10}{e_1}
\zindex{67.3}{10}{e_1'}
\zindex{35.5}{12.5}{\mbox{expand } e_1'}
\zindex{85}{12.5}{\mbox{collapse } e_1}
\zindex{10.5}{3.0}{e_1}
\zindex{110.5}{3.0}{e_1'}

==> pics/generic.tex <==
\thicklines
\put(10,10){\circle*{1}}
\put(25,15){\circle*{1}}
\put(25,5){\circle*{1}}
%\qbezier(10,10)(10,10)(25,15)
\put(10,10){\line(3,1){15}}
%\qbezier(10,10)(10,10)(25,5)
\put(10,10){\line(3,-1){15}}

\put(70,10){\circle*{1}}
\put(86,10){\circle*{1}}
%\qbezier(70,10)(70,10)(86,10)
\put(70,10){\line(1,0){16}}

\thinlines
\put(45,10){\vector(1,0){10}}

%\qbezier(10,10)(10,10)(5,8)
\put(10,10){\line(-5,-2){5}}
%\qbezier(25,15)(25,15)(29,19)
\put(25,15){\line(1,1){4}}
%\qbezier(25,5)(25,5)(31,4)
\put(25,5){\line(6,-1){6}}
%\qbezier(25,5)(25,5)(29,1)
\put(25,5){\line(1,-1){4}}

%\qbezier(70,10)(70,10)(65,8)
\put(70,10){\line(-5,-2){5}}
%\qbezier(86,10)(86,10)(90,14)
\put(86,10){\line(1,1){4}}
%\qbezier(86,10)(86,10)(92,9)
\put(86,10){\line(6,-1){6}}
%\qbezier(86,10)(86,10)(90,6)
\put(86,10){\line(1,-1){4}}

\normalsize
\zindex{9}{12}{w}
\zindex{25}{17.5}{u}
\zindex{25}{7}{v}
\zindex{70}{12}{ w}
\zindex{85}{12.5}{u'}

\zindex{50}{13}{\phi}

\scriptsize
\zindex{17.5}{14}{e}
\zindex{18}{9.3}{f}
\zindex{78}{12}{e'}


==> pics/generic2.tex <==
\thicklines
\put(10,10){\circle*{1}}
\put(25,15){\circle*{1}}
\put(25,5){\circle*{1}}

%\qbezier(10,10)(10,10)(25,15)
\put(10,10){\line(3,1){15}}
%\qbezier(10,10)(10,10)(25,5)
\put(10,10){\line(3,-1){15}}

\scriptsize
\zindex{12}{12}{a}
\zindex{12}{8}{c}
\zindex{22.5}{15.5}{b}
\zindex{22.5}{4.5}{d}

\put(70,10){\circle*{1}}
\put(86,10){\circle*{1}}

%\qbezier(70,10)(70,10)(86,10)
\put(70,10){\line(1,0){16}}

\thinlines
\put(45,10){\vector(1,0){10}}

%\qbezier(10,10)(10,10)(5,8)
\put(10,10){\line(-5,-2){5}}
%\qbezier(25,15)(25,15)(29,19)
\put(25,15){\line(1,1){4}}
%\qbezier(25,5)(25,5)(31,4)
\put(25,5){\line(6,-1){6}}
%\qbezier(25,5)(25,5)(29,1)
\put(25,5,){\line(1,-1){4}}

%\qbezier(70,10)(70,10)(65,8)
\put(70,10){\line(-5,-2){5}}
%\qbezier(86,10)(86,10)(90,14)
\put(86,10){\line(1,1){4}}
%\qbezier(86,10)(86,10)(92,9)
\put(86,10){\line(6,-1){6}}
%\qbezier(86,10)(86,10)(90,6)
\put(86,10){\line(1,-1){4}}

\normalsize
\zindex{9}{12}{\mathbf w}
\zindex{25}{17.5}{\mathbf u}
\zindex{25}{7}{\mathbf v}

\zindex{70}{12}{\mathbf w}
\zindex{85}{12.5}{\mathbf u'}

\scriptsize
\zindex{17.5}{14}{\mathbf e}
\zindex{17.5}{9.3}{\mathbf f}
\zindex{78}{12}{\mathbf e'}


==> pics/grapheg.tex <==
\thicklines
\scriptsize

\put(50,23){\circle*{1}}
\put(50,9){\circle*{1}}
\put(38,3){\circle*{1}}
\put(62,3){\circle*{1}}

\put(38,3){\line(1,0){24}}
\put(38,3){\line(3,5){12}}
\put(38,3){\line(2,1){12}}
\put(50,9){\line(0,1){14}}
\put(50,23){\line(3,-5){12}}
\put(50,9){\line(2,-1){12}}

\zindex{40}{1.5}{6}
\zindex{60}{1.5}{3}
\zindex{38}{6}{6}
\zindex{47.5}{21.5}{7}
\zindex{53}{21.5}{2}
\zindex{62}{6}{3}
\zindex{48}{9.7}{2}
\zindex{51}{7}{5}
\zindex{51.2}{11}{3}
\zindex{51.3}{17.5}{4}
\zindex{56}{4.5}{3}
\zindex{42.5}{7}{8}




==> pics/slide.tex <==
\thicklines
\put(70,10){\circle*{1}}
\put(85,10){\circle*{1}}
\put(70,10){\line(1,0){15}}
\put(85,10){\line(-1,2){4}}

\thinlines
\put(45,10){\vector(1,0){10}}

\put(85,10){\line(5,3){5}}
\put(85,10){\line(5,-3){5}}
\put(70,10){\line(-5,3){5}}
\put(64,10){\line(1,0){6}}
\put(70,10){\line(-5,-3){5}}

\scriptsize
\zindex{70}{7.5}{\As_v}
\zindex{77}{8}{\As_f}
\zindex{85}{7.5}{\As_w}
\zindex{84}{18}{\As_e}

\thicklines
\put(10,10){\circle*{1}}
\put(25,10){\circle*{1}}
\put(10,10){\line(1,0){15}}
\put(10,10){\line(1,2){4}}

\thinlines
\put(25,10){\line(5,3){5}}
\put(25,10){\line(5,-3){5}}
\put(10,10){\line(-5,3){5}}
\put(4,10){\line(1,0){6}}
\put(10,10){\line(-5,-3){5}}

\scriptsize
\zindex{10}{7.5}{\As_v}
\zindex{17}{8}{\As_f}
\zindex{25}{7.5}{\As_w}
\zindex{11.5}{18}{\As_e}


==> pics/slideloop.tex <==
\thicklines
\put(22,6){\circle{10}}
\put(22,11){\circle*{1}}
\put(22,11){\line(0,1){8}}

\put(78,6){\circle{10}}
\put(78,11){\circle*{1}}
\put(78,11){\line(0,1){8}}

\thinlines
\put(45,10){\vector(1,0){10}}

\put(22,11){\line(-1,1){4}}
\put(78,11){\line(-1,1){4}}
\put(22,11){\line(-6,1){6}}
\put(78,11){\line(-6,1){6}}

\zindex{24.5}{18}{\As_e}
\zindex{80.5}{18}{\As_e}

\zindex{22}{3}{\As_f}
\zindex{25.5}{12.5}{\As_v}

\zindex{78}{3}{\As_f}
\zindex{81.5}{12.5}{\As_v}


==> pics/zcollapse.tex <==
\thicklines
\put(10,10){\circle*{1}}
\put(25,10){\circle*{1}}
%\qbezier(10,10)(10,10)(25,10)
\put(10,10){\line(1,0){15}}

\thinlines
\put(45,10){\vector(1,0){10}}
\put(55,10){\vector(-1,0){10}}

%\qbezier(25,10)(25,10)(30,13)
\put(25,10){\line(5,3){5}}
%\qbezier(25,10)(25,10)(30,7)
\put(25,10){\line(5,-3){5}}

%\qbezier(10,10)(10,10)(5,13)
\put(10,10){\line(-5,3){5}}
%\qbezier(10,10)(10,10)(4,10)
\put(4,10){\line(1,0){6}}
%\qbezier(10,10)(10,10)(5,7)
\put(10,10){\line(-5,-3){5}}

\put(75,10){\circle*{1}}
%\qbezier(75,10)(75,10)(70,13)
\put(75,10){\line(-5,3){5}}
%\qbezier(75,10)(75,10)(69,10)
\put(69,10){\line(1,0){6}}
%\qbezier(75,10)(75,10)(70,7)
\put(75,10){\line(-5,-3){5}}

%\qbezier(75,10)(75,10)(80,13)
\put(75,10){\line(5,3){5}}
%\qbezier(75,10)(75,10)(80,7)
\put(75,10){\line(5,-3){5}}

\scriptsize
\zindex{3}{14}{s_1}
\zindex{2}{10}{s_2}
\zindex{3}{6}{s_3}
\zindex{12}{11.5}{l}
\zindex{23}{11.5}{1}
\zindex{32}{13}{r_1}
\zindex{32}{6}{r_2}

\zindex{83}{14}{lr_1}
\zindex{83}{6}{lr_2}
\zindex{68}{14}{s_1}
\zindex{67}{10}{s_2}
\zindex{68}{6}{s_3}
 

==> pics/zslide.tex <==
\thicklines
\put(70,10){\circle*{1}}
\put(85,10){\circle*{1}}
\put(70,10){\line(1,0){15}}
\put(85,10){\line(-1,2){4}}

\thinlines
\put(45,10){\vector(1,0){10}}

\put(85,10){\line(5,3){5}}
\put(85,10){\line(5,-3){5}}
\put(70,10){\line(-5,3){5}}
\put(64,10){\line(1,0){6}}
\put(70,10){\line(-5,-3){5}}

\scriptsize
\zindex{72}{8.5}{m}
\zindex{83}{8.5}{n}
\zindex{81.5}{13}{ln}

\thicklines
\put(10,10){\circle*{1}}
\put(25,10){\circle*{1}}
\put(10,10){\line(1,0){15}}
\put(10,10){\line(1,2){4}}

\thinlines
\put(25,10){\line(5,3){5}}
\put(25,10){\line(5,-3){5}}
\put(10,10){\line(-5,3){5}}
\put(4,10){\line(1,0){6}}
\put(10,10){\line(-5,-3){5}}

\scriptsize
\zindex{12}{8.5}{m}
\zindex{23}{8.5}{n}
\zindex{9.5}{14}{lm}
 

==> pics/zslideloop.tex <==
\thicklines
\put(22,6){\circle{10}}
\put(22,11){\circle*{1}}
\put(22,11){\line(0,1){8}}

\put(78,6){\circle{10}}
\put(78,11){\circle*{1}}
\put(78,11){\line(0,1){8}}

\thinlines
\put(45,10){\vector(1,0){10}}

\put(22,11){\line(-1,1){4}}
\put(78,11){\line(-1,1){4}}
\put(22,11){\line(-6,1){6}}
\put(78,11){\line(-6,1){6}}

\zindex{24.5}{13.5}{lm}
\zindex{80}{13.5}{ln}
\zindex{20.5}{9}{m}
\zindex{24}{9}{n}
\zindex{76.5}{9}{m}
\zindex{80}{9}{n}

 
